A KELT-TESS Eclipsing Binary in a Young Triple System Associated with a "Stellar String" Theia 301

HD 54236 is a nearby, wide common-proper-motion visual pair that has been previously identified as likely being very young by virtue of strong X-ray emission and lithium absorption. Here we report the discovery that the brighter member of the wide pair, HD~54236A, is itself an eclipsing binary (EB), comprising two near-equal solar-mass stars on a 2.4 d orbit. It represents a potentially valuable opportunity to expand the number of benchmark-grade EBs at young stellar ages. Using new observations of Ca2H&K emission and lithium absorption in the wide K-dwarf companion, HD 54236B, we obtain a robust age estimate of 225 +/- 50 Myr for the system. This age estimate and Gaia proper motions show HD 54236 is associated with Theia~301, a newly discovered local "stellar string", which itself may be related to the AB Dor moving group through shared stellar members. Applying this age estimate to AB~Dor itself alleviates reported tension between observation and theory that arises for the luminosity of the 90M_Jup star/brown dwarf AB Dor C when younger age estimates are used.

==> Referee_Response.tex <==
We would like to thank the referee for their positive, insightful comments and constructive suggestions on our manuscript. We have carefully reviewed their suggestions and modified the manuscript accordingly. Following is our response to each of the referee's suggestions; changes in the manuscript are shown in boldface type. We respectfully request that the paper be reconsidered now for publication in the Journal. 

Referee Report: 
Reviewer's Comments:
The authors present an interesting new eclipsing pre-main sequence binary. They have obtained lots of data for the system, which allows them to carry out a detailed analysis. Nevertheless, they need to do a bit more work to convince this referee that their results are solid, particularly with regard to accuracy of their estimate of the system's age.

Major Comments:
Comment:
The authors chose 2 chronometers to estimate the system age, why only 2? And, why those 2?

Response:
We have added two additional age verifications, one being isochrone fitting using the latest MIST stellar evolutionary models (newly added as Section 4.5.3), and secondly we have expanded Section 4.5.1 to include a much larger sample of benchmark cluster ages within the lithium abundance analysis. 


Comment:
In particular, I would like to see HD 54236B placed on the Hertzsprung-Russell diagram and its location compared with pre-main sequence evolutionary tracks and isochrones, and I would like to see a discussion of the gyrochronology dating method.

Response: 
We have followed the referee's recommendation by adding an HR diagram showing all three components of the HD 54236 system compared to the pre-main sequence (PMS) evolutionary models of Baraffe et al. (1998) as a new panel in Figure 16 and mentioned in Section 4.5. 


Comment:
In section 4.5.1 the authors considered four different age ranges to estimate probability, however the total probability of the figures they provide adds up to 0.53, suggesting that the probability of the age not being in any of those ranges is 0.47, larger than the probability in any of those particular age ranges. This does not make sense, so I recommend the authors work out in more detail, and/or describe more carefully, how they estimate their probabilities.

Response:
We have made the following changes to the 3rd paragraph of Section 4.5.1 in the manuscript to more carefully describe our methods for estimating our age probabilities: We have calculated the Lithium abundances for both the eclipsing binary HD 54236A and the tertiary HD 54236B following the methods of Soderblom 1993, and then these abundances are used to determine a best-fit age from the Sestito & Randich (2005) data for a large set of benchmark clusters. Figure 17 has been updated to reflect this more robust determination of our age estimates.  


Comment:
In Figure 11 the LiI resonance lines of both components in the EB are clearly seen. However, there is no figure that illustrates the LiI resonance line detection in HD 54236B, which is more critical to estimate the age of the system. A comparison similar to what is presented in Figure 18, but for lithium, would be worthwhile.

Response:
We have considered this recommendation but respectfully opt to retain the analysis as is. Figure 18 is showing the comparison of the Ca II H & K because the strength of their spectral features and the age of the stars do not have an empirical relationship like that which exists for lithium abundance and age. Figure 18 compares the presence of Ca H&K features in our target spectra to those present in other targets of known ages, effectively providing a Ca II H & K guided age estimate from targets with better constrained ages.


Comment:
More details should be given about the comparative analysis of Ca II H & K. How many stars were considered in each open cluster? What was the range of Teff? Was there any variability in CaII H & K observed?

Response:
More details were added to the manuscript section 4.5.2 on Ca II H & K including the stellar censuses and Teff ranges of the open clusters used for comparison. Being that the ANU multi epoch spectra do not contain Ca II H&K lines, we cannot compare CaII H&K variations from that dataset. We opted to utilize the ANU WiFeS spectrograph data both because our spectrum for HD 54236B was not absolutely flux calibrated and because the late spectral type of HD 54236B places it beyond the calibration of existing age-activity relationships (in this case the age versus R'HK relationship) which are based on single star angular momentum evolution. We instead compare our observed spectrum with suitable late-type standards from several young clusters whose age estimates are more constrained by the presence of several young members. 


Comment:
A closer look at Figure 17, focusing on the location of HD 54236 B, indicates that the constraints on the age are coming mainly from the following open clusters: alpha Per, Pleiades, M34, M7, and Coma Ber.

Response: 
Details were added to the Li section (4.5.1) including their stellar censuses and Teff ranges of the open clusters used for comparison, including alpha Per, Pleiades, M34, M7, and Coma Ber. We've also included additional information on calculating the Lithium Abundances following Soderblom (1993) and using them to find the best fit age from the Sestito and Randich (2005) cluster data that we had used before to better solidify the connection between the age of our system and to that of these clusters.  


Comment:
The connections between the AB Dor moving group and the Theia 301 stellar string are rather loose, and also the brown dwarf status of AB Dor C. It is a bit of a stretching to use results of this paper to constrain the age of this brown dwarf candidate. Note that 90 Mjup is clearly above the substellar-mass limit for solar metallicity. I recommend that the authors look for additional evidence to strengthen the connection between AB Dor and Theia 301, or else tone down their conclusions.

Response:
We appreciate the Referee for this comment, and the constructive changes it brought to our manuscript, which we summarize here:

Regarding the substellar mass limit for metallicity, and the brown dwarf candidate AB Dor C: 
It was not our intent to promote or question the matter of the stellar versus substellar status of AB Dor C, thus we have removed all references to AB Dor C as a brown dwarf, focusing instead on the question of the system's age as determined by us. 

Regarding the connection between AB Dor and Theia 301:
A similar type of connection has recently been made between other identified co-moving groups, e.g.: Ursa Major, and Theia 906, 908, 1008, 1009 & 1091 (Gange et al. 2020, RNAAS, 4, 92). In that case, the groups do not share any stars in common - rather, their argument is based on the similarity in the respective kinematics and isochronal ages of the populations. In this case, "fragmentation" occurs for a similar reason as with AB Dor and Theia 301 - one catalog ends within 80 pc, the other one starts at larger distances. Similarly, recently Stauffer et al. (2020, AJ, 160, 30) has established a likely connection between two stars and a 32 Ori moving group despite them being several tens of pc apart, again on the basis of the similarities in their respective kinematics and their ages. It can be difficult to establish a "definitive" connection between populations, but informed and dexterous inferences that they are related are advantageous. Arguably, having multiple stars in common in addition to sharing similar kinematics is a stronger argument for an overlap than the above two examples. We have added a bit of text to the beginning of the 5th paragraph of Section 5 to point the reader to some of these other related studies. 


Minor Comments: 
Comment:
It is hard to see anything in Figure 9. Please expand, and comment on the discrepancies between the data and the template.

Response: 
We enlarged both panels of Figure 9 for visual clarity. The Figure 9 caption was expanded to include the binary descriptor of HD 54236A and similarly, the tertiary descriptor of HD 54236B. We have also added a sentence to explain that the discrepancy between the target spectra and their respective templates are primarily caused by their difference in flux calibration, and that the spectral matching is done based on spectral features rather than overall shape.  

